Not all peaks are created equal: the early growth of Supermassive Black Holes

In this work, we use the constrained Gaussian realization technique to study the early growth of supermassive black holes (SMBHs) in cosmological hydrodynamic simulations, exploring its relationship with features of the initial density peaks on large scales, ~1 Mpc/h. Our constrained simulations of volume (20 Mpc/h)^3 successfully reconstruct the large-scale structure as well as the black hole growth for the hosts of the rare 10^9 Msun SMBHs found in the BlueTides simulation at z~7. We run a set of simulations with constrained initial conditions by imposing a 5 \sigma_0(R_G) peak on scale of R_G = 1 Mpc/h varying different peak features, such as the shape and compactness as well as the tidal field surrounding the peak. We find that initial density peaks with high compactness and low tidal field induce the most rapid BH growth at early epochs. This is because compact density peaks with a more spherical large scale matter distribution lead to the formation of high density gas clumps in the centers of halos, and thus boost early BH accretion. Moreover, such initially compact density peaks in low tidal field regions also lead to a more compact BH host galaxy morphology. This can explain the tight correlation between BH growth and host galaxy compactness seen in observations.

==> trash.tex <==


% \begin{figure}
% \begin{center}
% \includegraphics[width=1.0\columnwidth]{plots/large-scale-profile.png}
% \end{center}
%     \caption{Density contrast field $\delta_x$ smoothed over $\rm R_G$ = 0.9 Mpc/$h$ for the constrained simulations. $\delta_x$ is linearly extrapolated to $z = 0$.
%     }
%     \label{fig:large-scale-profile}
% \end{figure}

% \begin{figure}
% \begin{center}
% \includegraphics[width=0.9\columnwidth]{plots/large-scale-evolution.png}
% \end{center}
%     \caption{The evolution of the peak parameters on scale of $\rm R_G$ = 0.9 Mpc/$h$ for the 6 constrained simulations, with the initial compactness of $\rm x_d = 3.6$ (the solid lines) and $\rm x_d = 5.0$ (the dashed lines), and tidal field of $\epsilon = 15$ (the blue lines), $\epsilon = 34$ (the purple lines) and with $\epsilon = 58$ (the red lines) respectively.
%     In order to compare the density field across different redshifts,for each redshift the peak parameters are measured by linearly extrapolating the density field to $z=0$.
%     Top panel is the evolution of the height of the peak in unit of $\sigma_0 (\rm R_G)$. Note that the initial value for each simulation in this study is $\nu = 5 \sigma_0$ at $z=99$. 
%     The middle panel is the evolution of compactness $x_d$ in unit of $\sigma_2 (\rm R_G)$. The solid lines started with  $\rm x_d = 3.6 \sigma_2$ at $z=99$, while the dashed lines started with $\rm x_d = 5 \sigma_2$. The bottom panel shows the evolution of the tidal field magnitude in unit of km/s/Mpc, with initial value start with $\epsilon = 15, 34$ and 58 km/s/Mpc at $z=99$ respectively.
%     }
%     \label{fig:large-scale-evolution}
% \end{figure}



Each row gives the constrained simulations with different compactness for the intial density peak, with $\rm x_d$ = 3.6, 4.3 and 5.4 (in unit of $\sigma_2 (\rm RG)$) for the top, middle and bottom row separately.
Note that the ellipticity of the peaks are adapted accordingly to the corresponding $x_d$, as listed in Table~\ref{tab:paramlist}.


Growth history of the BH in the constrained simulations. From left to right column is the constrained simulation sets with compactness of averaged value $\rm x_d = 3.6$ and of $+1 \sigma$,$+2 \sigma$,$+3 \sigma$ variation respectively. The three lines in each panel correspond to the constrained simulation with different tidal field magnitude, with blue line for $\epsilon = 15$ km/s/Mpc, orange line for $\epsilon = 34$ km/s/Mpc, and green line for $\epsilon = 58$ km/s/Mpc.
\textit{Top panels:} The growth history of the BH mass. The gaps in the line indicate the merging event. During each merger event, only the more massive progenitor is traced and shown in the plot.
\textit{Middle panels:} The Eddington ratio $\dot{M}_{\rm BH}/M_{\rm Edd}$ of the BH growth as a function of time. Note that $M_{\rm Edd}$ is the function of $M_{\rm BH}$ (c.f. Equation~\ref{equation:Meddington}).
\textit{Bottom panels:} The gas density in the vicinity of the BH as a function of time. The gas density is in unit of $\rho_0$, which is the averaged matter density of the universe.


% \begin{figure}
% \begin{center}
% \includegraphics[width=0.9\columnwidth]{plots/MBH_Mstar.png}
% \end{center}
%     \caption{Scaling relation between $M_{\rm BH}$ with respect to the stellar mass in their host galaxy. The color and shape of the markers represent the peak compactness and tidal field magnitude of the constrained IC, with the same convention as Figure~\ref{fig:MBH-xd-epsilon}.
%     The blue shades are from the results of \textsc{BlueTides} simulation.
%     The brown dashed line give the observational result in the local universe from \citet{Reines2016}. 
%     The blue dashed line gives the scaling relation from study of \citet{Kormendy2013}.}
%     \label{fig:MBH_Mstar_relation}
% \end{figure}

% \begin{figure}
% \begin{center}
% \includegraphics[width=0.9\columnwidth]{plots/Mdot_sigma1.png}
% \end{center}
%     \caption{Caption}
%     \label{fig:Mdot_sigma1_relation}
% \end{figure}

% \begin{figure*}
% \begin{center}
% \includegraphics[scale=0.5]{plots/Mbh-sigma-BT3.png}
% ~
% \includegraphics[scale=0.5]{plots/bhm-sigma1-separate.png}
% \end{center}
% \caption{\textit{\textbf{Left plot:}} The relation between the BH mass and the central stellar mass surface density $\Sigma_1$. 
% The blue color gives the 2D histogram from \textsc{BlueTides}  simulation at $z=7$.
% The black dashed line gives the best linear fitting result of $\log M_{\rm BH}$ = 1.3 $\log$ ($\Sigma_1$) - 5.3, with intrinsic scatter of 0.17. 
% The colored scatter points give the result from the constrained simulations at $z=7$. The brown, purple, orange and red color of the marker represents compactness of the initial density peak $\rm x_d = 3.6$, 4.3, 5.0 and 5.8 respectively. The different tidal magnitude of the peak is represented by the shape of the marker for $\epsilon$ = 15 (triangle up), 34 (round), 58 (triangle down) km/s/Mpc.
% \textit{\textbf{Right plot:}} Split of the left panel plot to show the relation of $M_{\rm BH}$, $\Sigma_1$ with the peak parameter $\rm x_d$ (the left column) and $\epsilon$ (the right column) separately. The color and shape of the markers has the same convention as shown in the legend of the left panel. $\bullet$ {\tiziana Move top two panels of right figure after figure 9 and discuss this appropriately- as it shoes an overall summary of the results and use to discuss quantitative trends}}
% \label{fig:bhm-sigma1}
% \end{figure*}

% $\bullet$ \tiziana{You need to add the Mbh-M* relation in your simulations for the different parameters (same as in Fig 11 - and discuss whether the most massive BHs are off-set from the local relation}
% $\bullet$ \tiziana{Make a new section with the comparison with observations - this includes your left panel of Fig 11 and the Mbh-M* relation (find appropriate constraints)}
% $\bullet$ \tiziana{Run simulations further in redshift -it would be better to have results at z=6 too or at least start seeing the BH growth beyond the steep part of the cures - e.g. Fig 9.}
% $\bullet$ \tiziana{Run a simulation for a 6 sigma peak to investigate the relative BH growth in higher mass halos/density peaks (under the same conditions - 1 or 2-sigma compactness etc.. }


% \tiziana{This is the important section - this is where you should have a more systematic approach. You are narrowing
% the parameter study to just 2 parameters - but for those you should show perhaps: -2sigma, average and +2 sigma (for compactness and tidal field respectively). To the very very least
% you should add a -2sigma for compactness. Instead of showing all the the BH mass evolution for each just use the relative difference from the average. If you can add 1sigma or 3sigma all the better but at the very least use average and +/- 2 sigma. This would amount to just adding 1 simulation for compactness of -2sigma.
% You would have one plot where you keep compactness fixed and change (+/-2 sigma the tidal field and show the percentage difference in BH growth (I would not show mdot or other properties for those - then you would have a second plot for the relative difference in BH mass growth for average tidal field and +/-2 sigma compactness. The next plot would show the actual BH mass vs z - like you have it now - and would show the most massive black hole e.g. the blue lines you have for +2sigma compactness and -2sigma tidal field with associated accretion rate, density and entropy history.} 




In Figure~\ref{fig:large-scale-evolution}, we explore the evolution of the large scale properties of the density peak in different sets of constrained simulations. 
In particular, we trace the quantity of the peak significance $\nu$, compactness $\rm x_d$ and tidal field magnitude $\epsilon$ as a function of time, for the constrained simulation with the initial compactness $\rm x_d = 3.6$ (the solid lines) and $\rm x_d = 5.0$ (the dashed lines), and tidal field magnitude of $\epsilon = 15$, 34 and 58 Mpc/$h$, represented by the blue, purple and red lines respectively in the three panels of Figure~\ref{fig:large-scale-evolution}.

Since the peak parameters in unit of $\sigma_0(\rm R_G)$ and $\sigma_2(\rm R_G)$ are the variance of the linear density fluctuation at $z=0$, it is more natural to measure the quantities the density field at different redshifts by linearly extrapolating the density field to $z=0$, i.e., $\delta_0(\mathbf{x}) = \delta(\mathbf{x})/D(z)$, where $D(z)$ is the linear growth factor at redshift $z$.
All the peak parameters in  Figure~\ref{fig:large-scale-evolution} are measured on scale of $\rm R_G = 0.9$ Mpc/$h$, they all increase when going to lower redshift as a consequence of the non-linear evolution of the structure formation, since $\rm R_G$ is well below the linear scale at the redshift range we look at.

The top panel of Figure~\ref{fig:large-scale-evolution} gives the evolution of the peak height in unit of $\sigma_0 (\rm R_G)$. 
All the constrained simulations in this study started from the same initial value of the density peak: $\nu = 5 \sigma_0$ at $z=99$, and the peak height grows with time during the non linear structure formation, as the density fluctuation collapses to form halo and attracts the nearby matters to fall in the potential.
Comparison of the solid and dashed lines shows that, 
the density peak with smaller initial compactness grows faster then the one with higher initial $\rm x_d$, as they are more extended in the initial matter distribution compared to the peak with the same height but higher compactness (as shown in Figure~\ref{fig:params_separate}). 
For the peaks with the same compactness, the one with lower tidal field grows faster compared to their counterparts in higher magnitude of tidal field, as a consequence of more spherical large scale matter distribution surrounding the peak.

The middle panel of Figure~\ref{fig:large-scale-evolution} show the evolution of compactness $x_d$ of density peak.
in unit of $\sigma_2 (\rm R_G)$. The solid lines started with initial value of $\rm x_d = 3.6 \sigma_2$ at $z=99$, while the dashed lines started with $\rm x_d = 5 \sigma_2$. 
The compactness grows fast with time since it probes the evolution of the immediate surrounding of the density peak, (note that the corresponding kernels are the second order derivatives of the density peak, $\hat{H}_5 \sim \hat{H}_{10}$ are weighted by $k^2$).
Comparing between the blue, purple and red lines show that the density peaks with lower tidal field grow faster in the peak compactness. 
On the other hand, however, the density peaks with higher initial value of $\rm x_d$ has slightly slower growth in the compactness afterward, and would be caught up by the density peak with lower initial $\rm x_d$.
This might be a consequence of the lower significance of the density peaks with large initial $\rm x_d$ at later redshift.

The bottom panel of Figure~\ref{fig:large-scale-evolution} shows the evolution of the tidal field magnitude in unit of km/s/Mpc, with initial value start with $\epsilon = 15, 34$ and 58 km/s/Mpc for the blue, purple and red at $z=99$ respectively.
The evolution of the tidal field shows that the density peak with a lower or higher magnitude of the initial tidal will maintain to be lower or higher with time evolution.
While again the peak with higher initial compactness would grow slower in the tidal field magnitude.



\subsubsection{The growth of BH}

We divide the different simulations with respect to their initial compactness of the density peak, from left to right column are the simulation sets with initial $\rm x_d = 3.6$, 4.3, 5.0 and 5.8 (in unit of $\sigma_2$). The ellipticity of the density peaks are conditioned on $\rm x_d$ according to Table~\ref{tab:paramlist}.
For each panel in Figure~\ref{fig:BH-growth}, the solid lines represent the constrained simulations with the same compactness while different magnitude of tidal fields, with $\epsilon$ = 15, 34 and 58 km/s/Mpc for blue, orange and green lines respectively.
For each column, we can easily visualize the effect of the tidal field on the growth of SMBHs.

The first row of Figure~\ref{fig:BH-growth} shows the growth history of the black hole mass. 
The gaps shown in the plot are due to the BH merger event.
As also shown in Figure~\ref{fig:host-image}, there are several black holes in the substructures of the density peak that would contribute to the merger events.
For clarity, in Figure~\ref{fig:BH-growth} we only trace the more massive progenitor for each merger event.

The second row of Figure~\ref{fig:BH-growth} gives the corresponding Eddington accretion ratio of the BH $\lambda_{\rm Edd}$ smoothed over redshifts.
$\lambda_{\rm Edd}$ is defined as the ratio of the BH accretion rate with the upper limit of $\dot{M}_{\rm BH}$, which is $2\times \dot{M}_{\rm Edd} (M_{\rm BH})$ in our simulation (c.f. Equation~\ref{equation:Meddington}).
The third row of Figure~\ref{fig:BH-growth} shows the evolution of the gas density (smoothed over time) in the vicinity of the BH, which is used to calculate the Bondi accretion rate (c.f. Equation~\ref{equation:Bondi}). 
The gas density is in unit of the averaged matter density of the universe $\rho_0$.

The second and third panel show similar pattern in the time variation.
The surrounding gas density in the vicinity of BH is overall growing with time as the halo evolves and develop deeper gravitational potential in the center. 
AGN is fuelled by the surrounding high density gas and starts active accretion mode, as we can see in Figure~\ref{fig:BH-growth} that BH in high $\lambda_{\rm Edd}$ phase corresponds to the clumps in the gas density.
Meanwhile, AGN would dump part of its accretion energy to its surrounding, heating and clearing out the nearby fueling gas. 
This brings suppression to the growth of gas density and halt active accretion onto AGN itself.
Therefore the BH growth cannot always stay in high $\lambda_{\rm Edd}$ phase because of this self-modulation by AGN feedback.

Comparison between the blue, orange and green lines in each panel clearly shows that, for the density peaks with the same initial height, compactness and ellipticity, the peak with lower tidal field would have more rapid BH growth compared to their counterparts in higher tidal field. 
The BH growth favors quasi-spherically, low tidal field region of the density field, of which the gas quickly form high density in the center of the peak and boosts the early growth.  
% will eventually catch up in the BH growth

Also, comparing the BH growth in constrained simulations with different compactness indicates that the density peak with high initial compactness would also significantly boost the BH growth.
One of the reason is that density peak with a more compact initial distribution would form small halo earlier, and therefore result in an earlier seeding time of BH as well as form gas environment with higher density, which is crucial to the BH growth.



\subsubsection{Density profile of the BH host}
Comparing the halo profiles with different initial compactness $\rm x_d$ (as shown by the solid and dashed lines), we can see that the host halo of BH with a higher initial compactness $\rm x_d$ has a more cuspy density profile comparing to the one with lower initial $\rm x_d$, and also have higher density gas in the innermost region of the halo.

On the other hand, the density profiles of halo residing in different magnitude of the tidal field shows that, the halo within a lower tidal also has higher gas density in the central region compared to the one with larger tidal field, as a more spherical initial density distribution would help the in-falling gas to cusp in the halo center. 
For the constrained simulation with initial tidal field $\epsilon=15$ km/s/Mpc, the gas density in the innermost region of the halo is about 1 order of magnitude higher compared to the halo with the initial tidal field of $\epsilon=58$ km/s/Mpc.

As illustrated in Figure~\ref{fig:BH-growth}, the BH growth is sensitive to the surrounding gas density. 



\subsection{compactness of galaxy}
the blue color gives the 2D histogram of the $M_{\rm BH}$ versus $\Sigma_1$ extracted from \textsc{BlueTides} simulation at $z=7$, with the black dashed line giving the best fitting result of
\begin{equation}
    \log (M_{\rm BH}/M_{\odot}) = 1.3 \log (\Sigma_1/M_{\odot}/\rm{pkpc}^2) - 5.3
\end{equation}
The fitting has intrinsic scatter of 0.17. 
The colored points give the results extracted from all the constrained simulations at $z=7$, with the color representing different initial compactness of the density and the shape representing the initial tidal field magnitude (see the caption and legend for details).
The results from the constrained simulation match well with the distribution extracted from \textsc{BlueTides}.
The tight correlation between $M_{\rm BH}$ and $\Sigma_1$ suggests that the compactness of the galaxy morphology might have the same origin as that boost the growth of the early massive BH: high density gas environment in the central region of halo that both fuel the BH growth as well as the star formation.


% The constrain goal is to construct a density peak at the center of the 15 Mpc/$h$ simulation box, with the Gaussian characteristic scale $R_G = 0.6$ Mpc/$h$, peak height 5$\sigma_0(R_G)$, compactness $x_d = 2.5 \sigma_2(R_G)$, axial ratio $a^{2}_{12} = 2$ and  $a^{2}_{13} = 3$, $v_x = v_y = v_z = 0$ and tidal field $\omega = 2 \pi$, with magnitude $\epsilon = 20, 60, 100$ km/s/Mpc respectively.
% All the Euler angles are set to zero so that the resultant constrained field has principal axes aligned along the coordinates.

% \begin{figure*}
% \begin{center}
% \includegraphics[width=0.9\columnwidth]{realization.png}
% \end{center}
%     \caption{In this plot we give an example of applying CR to a Gaussian random field.
%     Each panel is 15 Mpc/$h$ per side, and 3 Mpc/$h$ of the slab width. The constraint position is at the original density peak. The significance of the peak was originally $3 \sigma_0(R_G)$ peak and then targeted/boosted to $5 \sigma_0(R_G)$ after the constrain.
%     The original tidal field magnitude of the peak was $\epsilon = 60$ km/s/Mpc.
%     The leftmost column show the original unconstrained field $\tilde{f} (\bf x)$ and the $\tilde{f}_G (\bf x)$ which is the $\tilde{f} (\bf x)$ field smoothed by a Gaussian filter with $R_G = 0.4$. 
%     The right three columns give the constrained fields with all the peak parameters the same except the tidal field magnitude $\epsilon$, with $\epsilon = 20, 60, 100$ km/s/Mpc for the second, third and fourth column respectively. 
%     The first row show the Ensemble mean field $\bar{f}_{es}(\bf x)$ added onto the original $\tilde{f} (\bf x)$ field, the second row is the density field after constraint $f(\bf x)$ = $\tilde{f} (\bf x)$ + $\bar{f}_{es}(\bf x)$, and the third row is the Gaussian smoothed constrained density field $f_G(\bf x)$ to show the density distribution on large scale.
%     }
%     \label{fig:realization example}
% \end{figure*}


% \footnote{see Appendix A for further discussion on the effects of box size}.

% Before we concentrate on the parameter space investigation for early BH growth, we illustrate the detailed distributions of the parameter values as well as the corresponding likelihood function of the parameter set (see also \cite{Bardeen1986} for the theory prediction).

% The full co-variance matrix of the parameter set is self-consistently calculated for the simulations we discuss in this section.\yy{this sentence does not sound concrete.}
% As mentioned in Section 2.2, the order and variance of the peak parameters can be estimated via their corresponding spectral moment (c.f. Equation~\ref{equation:spectral_moment}).
% However, spectral moment is calculated for the overall density field, while we need the distribution of the peak parameter for 5$\sigma$ peaks (i.e., conditioned on $\nu = 5 \sigma_0$). 

% We recover the distribution of the peak parameters conditioned on 5$\sigma$ peaks in our simulation box size of 20 Mpc/$h$ directly. In particular, we generate a large set (30,000) random realizations of initial conditions on which we impose the $5 \sigma_0$ peak constraint on a random position. We then read out the resultant density peak parameters on scale of $\rm R_G = 1$ Mpc/$h$ to get the overall distribution.
% Note that the computational cost for generating this large number of constrained ICs is pretty minimal (only tens of core hours).
% \tiziana{I am not sure what to do with the sentence below -
% becoming so specific... perhaps add it later after you show the other params?}
% However, we note that the distribution of some field properties, such as the peculiar velocity of the peak, can be largely effected by the box size of the simulation because the variation of $\sigma_{-1}$ is mostly contributed by scales larger than our box size (see Appendix A for details).
% \tiziana{just braketing the sentence above}


% figures

% \begin{table*}
% \centering
% \makebox[1.8\columnwidth][c]{
% \begin{tabular}{ccccccccc}
% \toprule
% \multicolumn{1}{c}{$f_{\rm 0,G}$} & \multicolumn{3}{c}{$f_{\rm 2,G}$} & \multicolumn{2}{c}{$T_{\rm G}$} & \multicolumn{3}{c}{$V_{\rm G}$} \\
% \cmidrule(lr){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-9}
% $\nu$ ($\sigma_0$) & $\rm x_d$ ($\sigma_2$) & $\rm a^2_{12}$ & $\rm a^2_{13}$  & $\epsilon$ (km/s/Mpc) & $\omega$ & $v_x$ (km/s) & $v_y$ (km/s) & $v_z$ (km/s) \\\midrule
% 5 & 2.2 ($-2\sigma$) & 1.7  & 2.8  & 8 ($-3\sigma$)  & 1.5$\pi$ & 0 & 0 & 0 \\
%   & 3.6 (ave)        & 1.54 & 2.1  & 15 ($-2\sigma$) & 1.5$\pi$ & & & \\
%   & 4.3 ($+1\sigma$) & 1.43 & 1.9 & 34 (ave) & 1.5$\pi$ & & & \\
%   & 5.0 ($+2\sigma$) & 1.35 & 1.7 & 58 ($+2\sigma$) & 1.5$\pi$ & & &\\
%   & 5.8 ($+3\sigma$) & 1.29 & 1.6 &    &  & & & \\
% \bottomrule
% \end{tabular}
% }
% \caption{List of the peak parameters we explore in our constrained simulation.}
% \label{tab:paramlist}
% \end{table*}



% Table --------------------------------------------
% \begin{table}
% \centering
% \begin{tabular}{llllllllll}
%     \hline
%      &$\nu$ & $\rm x_d$ & $a_{12}^2$ & $a_{13}^2$ & $v_x$ & $v_y$ & $v_z$ & $\epsilon$ & $\omega$ \\
%      \hline
%      &$\sigma_0$ & $\sigma_2$ &  &  & km/s & km/s & km/s & rad & km/s/Mpc \\
%     %  &[$\sigma_0$] & [$\sigma_2$]& & &[km/s] &  & [rad] \\
%      \hline
%     uncons & 3.6 & 3.2 & 2.7 & 3.8 & 5 & 27 & 43 & 40 & 5.6 \\
%     \textsc{BT-BigBH} & 4.8 & 5.7 & 1.4 & 2.0 & 23 & -73 & -8 & 34 & 3.9 \\
%     \textsc{BT-BigHalo} & 6.0 & 4.5 & 2.0 & 3.0 & 17 & -13 & 115 & 60 & 4.5 \\
%     \hline
% \end{tabular}



is a linear functional of the $f(\mathbf x)$ field.
to have specific value $c_i$ at position $\mathbf x = \mathbf r_c$.
We only consider linear functionals of the field, that the constraint value $c_i$ is obtained by convolving the $f(\mathbf x)$ field with some kernel $H_i(\mathbf x, \mathbf r_c)$ leading to the convolved field value at position $\mathbf r_c$. 
Therefore, $C_i$ can be written in the form 
